Hidden Figures in Software Engineering: A Replication Study Exploring Undergraduate Software Students' Awareness of Distinguished Scientists from Underrepresented Groups

Technology is a cornerstone of modern life, yet the software engineering field struggles to reflect the diversity of contemporary society. This lack of diversity and inclusivity within the software industry can be traced back to limited representation in software engineering academic settings, where students from underrepresented groups are often stigmatized despite the field's rich history of contributions from scientists from diverse backgrounds. Over the years, studies have revealed that women, LGBTQIA+ individuals, and Black students frequently encounter unwelcoming environments in software engineering programs. However, similar to other fields, increasing awareness of notable individuals from marginalized backgrounds could inspire students and foster a more inclusive environment. This study reports the findings from a replicated global survey with undergraduate software engineering students, exploring their knowledge of distinguished scientists from underrepresented groups. These findings show that students have limited awareness of these figures and their contributions, highlighting the need to improve diversity awareness and develop educational practices that celebrate the achievements of historically marginalized groups in software engineering. Index Terms-EDi in software engineering, software engineering education, diversity.

==> tables/targets.tex <==
\begin{table}[h!]
\caption{Targets for Fairness Testing}
\centering
\label{tab:fairness_testing_targets}
\begin{tabularx}{\linewidth}{p{2cm} X}
\toprule
\textbf{Target} & \textbf{Evidence Examples} \\ \hline

\textbf{\textit{Testing for Diversity and Inclusivity}} & \textit{``We use examples of people with reduced mobility and other types of conditions to ensure fair inclusion in recognition.''} (P6) \newline \\
& \textit{``We had to introduce people of different skin tones and watched how the algorithm responded to each of them.''} (P7) \newline \\
& \textit{``We seek people from different ethnicities, races, and genders to build a more diverse dataset.''} (P14) \newline \\
& \textit{``We tried to set up a database that reflects Brazil's ethnic diversity to improve recognition.''} (P13) \\ \hline

\textbf{\textit{Testing for Model Consistency}} & \textit{``We started with exploratory tests initially, experimenting and seeing the answers that generated it.''} (P4) \newline \\
& \textit{``We need to assemble this database so that the algorithm learns from those data, as bias can occur when data does not reflect reality.''} (P9) \newline \\
& \textit{``We tried to find out if the AI's responses were consistent, or if it had variables that weren't in the original data.''} (P16) \newline \\
& \textit{``We tested the modeling capacity of the model, verifying if it can present good results with data never seen.''} (P17) \\ \hline

\textbf{\textit{Testing for Data Representation and Balancing}} & \textit{``We greatly tested data balancing and how it influenced the results of the model.''} (P15) \\
& \textit{``We tried to ensure that the data we use to train are representative and balanced, seeking to avoid embedded bias.''} (P19) \newline \\
& \textit{``We tested data balancing to see if the classes are well distributed, this is critical to avoiding bias.''} (P21) \newline \\
\bottomrule
\end{tabularx}
\end{table}

